Worst of Both Worlds: Biases Compound in Pre-trained Vision-and-Language Models

Numerous works have analyzed biases in vision and pre-trained language models individually - however, less attention has been paid to how these biases interact in multimodal settings. This work extends text-based bias analysis methods to investigate multimodal language models, and analyzes intra- and inter-modality associations and biases learned by these models. Specifically, we demonstrate that VL-BERT (Su et al., 2020) exhibits gender biases, often preferring to reinforce a stereotype over faithfully describing the visual scene. We demonstrate these findings on a controlled case-study and extend them for a larger set of stereotypically gendered entities.

==> assocations.tex <==
\begin{table*}[t]
\small
\centering
\begin{tabular}{l c l l l}

     \toprule
     \vspace{1mm} \multirow{2}{*}{Source} & \multicolumn{2}{c}{To compute $P(E|g)$} & \multicolumn{2}{c}{To compute $P(E|g_N)$}\\ 
     & \multicolumn{1}{c}{Visual Input} & \multicolumn{1}{c}{Language Input}    & \begin{tabular}[c]{@{}c@{}}Modified\\Component\end{tabular} & \multicolumn{1}{c}{New Value}         \\
     \cmidrule(lr){2-3} \cmidrule(lr){4-5} \vspace{1mm}
     \begin{tabular}[c]{@{}l@{}}Visual-Linguistic\\ Pre-training\\ (S\ref{subsubsec:pt})\end{tabular} & \textcolor{red}{\xmark} & The \texttt{man} is drinking \texttt{beer} & Model & Text-only LM \\
     
     \bottomrule
     
\end{tabular}
\caption{}
\label{tab:methods-table}
\end{table*}


==> drinks.tex <==
Our analysis so far has utilized our framework for measuring relational knowledge to measure gender bias for different entities. We do this by comparing association scores between entities and the gender of the agent. However, we also want to know how our methodology can be used to measure relational knowledge for entities with other kinds of information units. We focus on alcoholic beverages as our entities, and examine how scene information and the choice of verb can influence masked probabilities extracted from the visual-linguistic model.

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figs/drinks-verbs.png}
    \caption{Language association scores $S_L(E, u)$ between drinks ($E$) and action words for consuming drinks $u \in \{ \textit{drinking, chugging, sipping} \}$}
    \label{fig:drinks-verb}
\end{figure}
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figs/drinks-scenes.png}
    \caption{Language association scores $S_L(E, u)$ between drinks ($E$) and scenes where drinks are consumed $u \in \{ \textit{bar, nightclub, pub} \}$}
    \label{fig:drinks-scene}
\end{figure}

We choose five alcoholic beverages - \textit{beer, wine, whiskey, champagne} and \textit{cocktails}.  To investigate the effect of verb choice in the language caption, we create a template caption, \texttt{The person is \texttt{[VERB]} \texttt{[DRINK]} .}. We choose three verbs - \textit{drinking, chugging, sipping} - which represent three different styles of consuming alcohol. For our information-neutral form of the verb, we use the template caption \texttt{The person has a \texttt{[DRINK]} }. For the visual input, we once again collect a balanced set of images for each drink, which consists of 6 images each of men and women with the drink. We compute language association scores between the drinks and the verbs, and plot them in Figure~\ref{fig:drinks-verb}. We see that most of the drinks have positive association scores with all of the verbs, with \textit{champagne} and \textit{chugging} being the only negatively associated pair. We also note that the most associated verb varies for each drink. Beer is most associated with \textit{chugging}, whereas wine, champagne and cocktail are far more associated with \textit{drinking} and \textit{sipping} than \textit{chugging}. 


We can similarly measure relational knowledge between drinks and scene information in the language caption. We use the template caption, \texttt{The person in the [SCENE] has a [DRINK] .}, and choose three scenes where alcohol is typically consumed - \textit{bar, pub, nightclub}. For the information-neutral form of the scene, we omit the clause pertaining to the scene. Using the same same set of images for each drink, we compute language association score between the drinks and the scenes, which are visualized in Figure~\ref{fig:drinks-scene}. We see similar trends here, where beer and whiskey are strongly associated with \textit{bars} and \textit{pubs}, whereas champagne and cocktail are most associated with \textit{nightclubs}. The strongly negative association scores for whiskey with nightclubs suggests that the model does not believe anyone drinks wine at a club.


==> ethical.tex <==
Gender is not binary, but this work performs bias analysis for the terms ``male" and ``female" -- which are traditionally proxies for cis-male and cis-female.  In particular, when images are used of male and female presenting individuals we use images that self-identify as male and female.  We avoid guessing at gender presentation and note that the biases studied here in this unrealistically simplistic treatment of gender pose even more serious concerns for gender non-conforming, non-binary, and trans-sexual individuals.  A critical next step is designing more inclusive probes, and training (multi-modal) language models on more inclusive data. We welcome criticism and guidance on how to expand this research.  Our image based data suffers from a second, similar, limitation on the dimension of race. All individuals self-identified as ``white" or ``black", but a larger scale inclusive data-collection should be performed.


==> vcr_examples.tex <==
\begin{table*}[t]
\small
\centering
\begin{tabular}{c c p{12cm}}

     \toprule
     Entity & Input Types &\quad\quad Language Inputs \\ 
     \midrule
     \multirow{2}{*}{Purse} & Template & \quad\quad she is carrying a \textit{purse} .\\
     \cmidrule{2-3}
     & VCR Rationales & \begin{itemize}\vspace{-6mm}
     \itemsep-0.5em
         \item she is standing on the curb with her \textit{purse} out .
         \item she is carrying her \textit{purse} and holding her stomach as if she ' s hungry .
         \item she ' s in a hotel hallway and she ' s looking down so she might be looking in her \textit{purse} for her key . \vspace{-4mm}
     \end{itemize} \\     
     \midrule
     \multirow{2}{*}{Briefcase} & Template & \quad\quad she is carrying a \textit{briefcase} .\\
     \cmidrule{2-3}
     & VCR Rationales & \begin{itemize}\vspace{-6mm}
     \itemsep-0.5em
         \item she is wearing all formal and holding a \textit{briefcase} .
         \item she ' s standing in the background holding a \textit{briefcase} , as if waiting her turn .
         \item she is holding a \textit{briefcase} . which is used in work areas . she also looks to be in a hurry like she needs to get to work .\vspace{-4mm}
     \end{itemize} \\     
     \midrule  
     \multirow{2}{*}{Apron} & Template & \quad\quad she is wearing a \textit{apron} .\\
     \cmidrule{2-3}
     & VCR Rationales & \begin{itemize}\vspace{-6mm}
     \itemsep-0.5em
         \item she is wearing an \textit{apron} and standing next to a table outside a cafe .
         \item there are espresso machines , and desserts like you would find in a coffee shop , and she is wearing an \textit{apron} with a name tag .
         \item she is wearing what looks like a white bonnet and \textit{apron} , so she ' s likely the maid .\vspace{-4mm}
     \end{itemize} \\     
     \midrule  
     \multirow{2}{*}{Suit} & Template & \quad\quad she is wearing a \textit{suit} .\\
     \cmidrule{2-3}
     & VCR Rationales & \begin{itemize}\vspace{-6mm}
     \itemsep-0.5em
         \item she has a nice \textit{suit} on and has luggage beside her .
         \item her \textit{suit} is clean and sharp and her haircut looks crisp as well .
         \item she is in a \textit{suit} and people do not usually carry on conversations on a plane unless it is important .\vspace{-4mm}
     \end{itemize} \\     
     \bottomrule
     
\end{tabular}
\caption{Examples from the VCR rationales (and the template caption for reference) for various entities, that we used in our analysis in Section 5.2. We have presented only the \textit{female} versions of the caption, but we also create male and gender-neutral versions by replacing the pronouns.}
\label{tab:vcr-examples}
\end{table*}

